Algorithms for the Diverse-k-SAT problem: the geometry of satisfying assignments

Given a $k$-CNF formula and an integer $s$, we study algorithms that obtain $s$ solutions to the formula that are maximally dispersed. For $s=2$, the problem of computing the diameter of a $k$-CNF formula was initiated by Creszenzi and Rossi, who showed strong hardness results even for $k=2$. Assuming SETH, the current best upper bound [Angelsmark and Thapper '04] goes to $4^n$ as $k \rightarrow \infty$. As our first result, we give exact algorithms for using the Fast Fourier Transform and clique-finding that run in $O^*(2^{(s-1)n})$ and $O^*(s^2 |\Omega_{F}|^{\omega \lceil s/3 \rceil})$ respectively, where $|\Omega_{F}|$ is the size of the solution space of the formula $F$ and $\omega$ is the matrix multiplication exponent. As our main result, we re-analyze the popular PPZ (Paturi, Pudlak, Zane '97) and Sch\"{o}ning's ('02) algorithms (which find one solution in time $O^*(2^{\varepsilon_{k}n})$ for $\varepsilon_{k} \approx 1-\Theta(1/k)$), and show that in the same time, they can be used to approximate the diameter as well as the dispersion ($s>2$) problems. While we need to modify Sch\"{o}ning's original algorithm, we show that the PPZ algorithm, without any modification, samples solutions in a geometric sense. We believe that this property may be of independent interest. Finally, we present algorithms to output approximately diverse, approximately optimal solutions to NP-complete optimization problems running in time $\text{poly}(s)O^*(2^{\varepsilon n})$ with $\varepsilon<1$ for several problems such as Minimum Hitting Set and Feedback Vertex Set. For these problems, all existing exact methods for finding optimal diverse solutions have a runtime with at least an exponential dependence on the number of solutions $s$. Our methods find bi-approximations with polynomial dependence on $s$.

==> app_schsum.tex <==
\section{\sch-based algorithm for the sum dispersion measure: Proof of \Cref{thm:sch-for-sumdisp}.}
\label{app:schsum}
To start with, we restate \Cref{thm:sch-for-sumdisp}. 
\schopts*
To prove this theorem, we show that \sch's algorithm can be modified to be a farthest point oracle for $\sumd$. 
\begin{lemma} \label{lem:schFarthestSum}
    Consider a local search algorithm $\LS_{\alpha, c}$. Then, for every $0 < \delta \leq \frac{2(1+\alpha)}{c-1}$, there exists an algorithm  running in time $s^2 \cdot n^{O(1)} \cdot \frac{2^n c^{R}}{\binom{n}{R} }$, where $R=\floor{\frac{\delta n}{2(1+\alpha+\delta)}}$ that takes as input $\f$ and a multi-set $S \subseteq \{0,1\}^n$ of size $s$ and if $\f$ is satisfiable, outputs $z^* \in \Om$ such that $\sumd(z^*, S) \geq \left(1-\delta\right) \cdot \max_{z' \in \Om} \sumd(z', S)$ with probability at least $1-2^{-2n}$. 
 \end{lemma}

 
 \begin{proof}
    Consider the following algorithm, that in line 6, uses the $\ALS_{\alpha, c, \delta}$ subroutine defined in the proof of \Cref{lem:anchor:sch}. 
    
    \begin{algorithm}[H] \label{alg:schFarthestSum}
 \KwIn{A $k$-CNF formula $\f$, $S \subseteq \{0,1\}^n, |S|=s$}
 \KwOut{$z^* \in \Om$ with $\sumd(S,z^*) > \left(1-\delta\right) \max_{z \in \Om}\sumd(S,z)$ if $\f$ is satisfiable, $\perp$ otherwise.}
 Set $z^*=\perp, D=0$. \\
 \SetKwFor{RepeatTimes}{repeat}{times:}{endfor}
 \For{$r \in \{0,1,2,\dots, n\}$}{
    \For{$z \in S$}{
        Let $t:=\min\left\{ \floor{\frac{\delta r}{1+\alpha}}, R\right\}$ \\
        \RepeatTimes{$n^{O(1)} \cdot |A_{r-t,r+t} (z)|$}{
        $u:=\ALS_{\alpha, c ,\delta}(\f,z,r)$\\
    \If{$u$ satisfies $\f$ and $\sumd(S,z^*) > D$}{
        $z^* \gets u, D \gets \sumd(S,u)$.
    }
    
    }
    }
    }
    Output $z^*$
 \caption{\textsf{\sch-Farthest-Sum}}
\end{algorithm}

    
     Suppose that there exists $z_0 \in \Om$ with $\sumd(z_0, S) = r$. Then, there must exist $z \in S$ such that $r':=d_H(z, z_0) \leq r/s$. Now, suppose that $\ALS_{\alpha, c ,\delta}(\f,r',z)$ outputs $z^* \in \Om$ such that $d_H(z^*, z_0) \leq \delta r'$. The triangle inequality then implies that $$\sumd(z^*, S)= \sum_{z \in S} d_H(z^*,z) \geq \sum_{z \in S} \left( d_H(z_0,z)-d_H(z^*, z_0)\right) \geq r-\delta s r' \geq \left(1-\delta \right)r \; .$$
    
    $\ALS_{\alpha,\delta}(\f, z, r')$ outputs such a $z^*$ if $y$, the starting assignment it samples, $y$ is within distance $t$ of $z_0$, This happens with probability at least $\frac{\binom{n}{t}}{|A_{r-t , r+t}(z)|}$
    Hence, it is sufficient to call $\LS_{\alpha, \delta}(\f, z, r')$ $n^{O(1)} \cdot \frac{|A_{r'-t , r'+t}(z)| c^t}{\binom{n}{t}  }$ (where $t$ is the value chosen corresponding to $r'$ by $\ALS_{\alpha, c ,\delta}$) times for each $r' \in \{0,1,2,\dots, n\}$ and $z \in S$, to ensure that the algorithm outputs $z^* \in \Om$ with $\sumd(S,z^*) \geq \left(1-\delta\right) \cdot \max_{z \in \Om} \sumd(z,S)$ with probability $1-2^{-2n}$, and the reminder of this proof (bounding the running time) is identical to the proof of \Cref{lem:anchor:sch}. The factor of $s^2$ in the running time bound arises from the fact that computing $\sumd(\cdot, \cdot)$ takes at most $s n$ time and due to the fact that we iterate over all $s \in S$ in line 3.  
 \end{proof}

\subsubsection*{Proof of \Cref{thm:sch-for-sumdisp}}
The proof of \Cref{thm:sch-for-sumdisp} is similar to that of \Cref{thm:ppz-for-sumdisp}. We use the algorithm $\textsf{\sch-Farthest-Sum}$ (\Cref{lem:schFarthestSum}) as a $(1-\delta)$-farthest point oracle, in the algorithm defined by \Cref{lem:sumdispersion}. The approximation, running time guarantees and the range of $\delta$ that the two algorithms handle follows from the bounds stated in~\Cref{lem:schFarthestSum} for $c=k, \alpha=1$ and $c=k-1, \alpha=3$. 
